Linear Programming Based Near-Optimal Pricing for Laminar Bayesian Online Selection

The Bayesian online selection problem aims to design a pricing scheme for a sequence of arriving buyers that maximizes the expected social welfare (or revenue) subject to different structural constraints. Inspired by applications with a hierarchy of service, this paper focuses on the cases where a laminar matroid characterizes the set of served buyers. We give the first Polynomial-Time Approximation Scheme (PTAS) for the problem when the laminar matroid has constant depth. Our approach is based on rounding the solution of a hierarchy of linear programming relaxations that approximate the optimum online solution with any degree of accuracy, plus a concentration argument showing that rounding incurs a small loss. We also study another variation, which we call the production-constrained problem. The allowable set of served buyers is characterized by a collection of production and shipping constraints that form a particular example of a laminar matroid. Using a similar LP-based approach, we design a PTAS for this problem, although in this special case the depth of the underlying laminar matroid is not necessarily a constant. The analysis exploits the negative dependency of the optimum selection rule in the lower levels of the laminar family. Finally, to demonstrate the generality of our technique, we employ the linear programming-based approach employed in the paper to re-derive some of the classic prophet inequalities known in the literature -- as a side result.

==> tex/LP-old.tex <==
\label{sec:lp-prophet}
The benefits of our linear programming approach for the online Bayesian selection problem are two-fold. So far, we have seen our LPs give us a systematic way of describing the optimum online benchmark and its relaxations, which can be easily generalized to other combinatorial domains (e.g. matroids). In this section, we show some further applications of this approach in the classic single-item prophet inequality problem (defined formally in \Cref{sec:prophet}).  We show how to use this LP to design approximate pricing mechanisms with respect to the optimal offline in a \emph{modular way}, and therefore re-deriving simpler proofs for a couple of already existing prophet inequalities. We believe this approach can be useful for other settings as well, which we leave as future research directions. For the ease of exposition, we focus on non-atomic distributions. The case of general distributions can be easily handled by adding randomized tie-breaking to our mechanisms in a straightforward fashion.

\subsection{Classic single-item Prophet inequality problem}
\label{sec:prophet}
In single item prophet inequality problem, a seller is interested in selling an item to a sequence of $n$  arriving buyers. Each buyer $i$ has a value $v_i$ for the item. This value is independently drawn from a distribution $\Fi{i}$. Buyers arrive one by one and reveal their values. Upon the arrival of a buyer, the seller decides whether to sell the item or move on to the next buyer. The goal is to maximize the expected value of the selected buyer. We consider the setting where the sequence of distributions $\Fi{1},\Fi{2},\ldots,\Fi{n}$ is picked by an oblivious adversary up front. We assume the seller knows the distributions in advance but does not know the order in which the buyers arrive  (an important distinction with previous sections of our paper). 

In contrast to previous sections, in which the goal was to design policies that approximate the optimum online benchmark, here we focus on obtaining prophet inequalities, where the goal is to design online policies that are competitive with respect to the optimum offline (or omniscient prophet) benchmark. In the single-item problem, this benchmark is simply equal to $\Ex{\underset{i\in[n]}{\max}~{v_i}}$.

\subsection{LP characterization of the optimum online benchmark} 
Let $\pi:[n]\rightarrow [n]$ be the arrival order of the buyers such that at each time $t=1,\ldots,n$ buyer $\pi(t)$ arrives. Now, for an ordering $\pi$ over the buyers, let $\opton(\pi)$ be the optimum online mechanism knowing $\pi$. We seek to find a linear programming characterization for $\opton(\pi)$ for a fixed $\pi$. Note that using a simple backward induction one can find such an optimum policy; However, the introduced LP sheds more insight on the structure of this policy and helps us with designing approximate policies with respect to the optimum offline (i.e. prophet inequalities).

To write down the linear program for the single item prophet inequality problem, similar to (\ref{eq:lp-optimal}), let $\x{t}(v)$ denote the probability that the policy allocates the item to the buyer arriving at time $t$ conditioned on the event that the value of this buyer is equal to $v$. Our linear programming has variables $\x{t}(v)$ for every $t\in [n]$ and every $v\in \textrm{supp}(\Fi{\pi(t)})$, where $\textrm{supp}(.)$ denotes the support of its input distribution. \footnote{In the case of non-atomic distributions, this LP is essentially a continuous program with uncountably many variables. In the case of discrete distributions, the LP has finitely many variables.} We then try to impose constraints on these variables to guarantee that the solution of the LP is  online implementable, without losing anything in the expected allocated value. Formally speaking, consider the following linear program, which we denote by $\lpon(\pi)$:


\begin{align*}
\raisetag{85pt}
\label{eq:lp-opt-on}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle \sum_{t=1}^{n}\Exv{v_{\pi(t)}\sim\Fi{\pi(t)}}{v_{\pi(t)}\cdot \x{t}(v_{\pi(t)})}  & &\tag{\texttt{LP-ONLINE}($\pi$)}\\
\text{subject to}& \displaystyle \x{t}(v)\leq 1-\sum_{t'<t}\Exv{v_{\pi(t')}\sim\Fi{\pi(t')}}{\x{t'}(v_{\pi(t')})} ,&~~~~~~~\forall v\in \textrm{supp}(\Fi{\pi(t)}),~t=2,\ldots,n\\
& \x{1}(v)\leq 1, &~~~~~~~\forall v\in \textrm{supp}(\Fi{\pi(1)})\\
& \x{t}(v)\geq 0, &~~~~~~~\forall v\in \textrm{supp}(\Fi{\pi(t)}),~t=1,\ldots,n
\end{array}
\end{align*}

It is not hard to see that every feasible online policy induces a feasible solution for \ref{eq:lp-opt-on}, by setting $\x{t}(v)$ to be the allocation probabilities of this policy. In fact, no allocation happens at time $t$ if the item has been allocated at some time $t'<t$. Therefore, by taking an expectation with respect to the buyer values arriving at times $t'=1,\ldots, t-1$, $\x{t}(v)$ will be at most equal to $1-\sum_{t'<t}\Exv{v_{\pi(t')}\sim\Fi{\pi(t')}}{\x{t'}(v_{\pi(t')})}$. More interestingly, the converse is also true. While we can prove the converse by applying \Cref{prop:adaptive-pricing} and slightly modifying the LP, we can also prove it directly. In order to be self-contained, we provide the direct proof here.

\begin{proposition}
\label{prop:rounding-exact}
Given any feasible assignment $\{\x{t}(v)\}$ for \ref{eq:lp-opt-on}, there exists a feasible online policy with an expected allocated value equal to the objective value of the LP under $\{\x{t}(v)\}$.
\end{proposition}
\begin{proof}{Proof.} Define $q_t\triangleq 1-\sum_{t'<t}\Exv{v_{\pi(t')}\sim\Fi{\pi(t')}}{\x{t'}(v_{\pi(t')})}$ for $t\geq 2$, and $q_1\triangleq 1$. Consider the following randomized rounding policy: at time $t\geq 1$, if the item has already been allocated do nothing. If it has not yet been allocated,  upon realizing the value $v_{\pi(t)}$ flip an independent coin with heads probability  of $\frac{\x{t}(v_{\pi(t)})}{q_t}$. Now, if the coin flips heads allocate the item and terminate. Otherwise, continue to the next buyer. 

Clearly the above policy is online and feasible, i.e. it sells the item to only one buyer. To compare its expected allocated value with the objective value of the LP under the assignment $\{\x{t}(v)\}$, we first claim that $q_t$ is equal to the probability that this randomized policy reaches time $t$, i.e. with probability $q_t$ the policy does not sell the item to any buyer arriving before time $t$. We prove this claim by induction. Clearly $q_1=1$ satisfies this property. As the induction hypothesis, suppose the policy reaches time $t\geq 2$ with probability $q_t$. To prove the inductive step, we have:
\begin{align*}
\Pr{\textrm{reaching time $t+1$}}&=\Pr{\left( \textrm{reaching time $t$} \right)\&\left(\textrm{no allocation at time $t$}\right)}\\
&=\Pr{\textrm{no allocation at time $t$}|\textrm{reaching time $t$}}\cdot q_t\\
&=\Exv{v_{\pi(t)}\sim\Fi{t}}{\Pr{\textrm{no allocation at time $t$}|\left(\textrm{reaching time $t$}\right)~\&~v_{\pi(t)}}}\cdot q_t \\
&=\Exv{v_{\pi(t)}\sim\Fi{t}}{1-\frac{\x{t}(v_{\pi(t)})}{q_t}}\cdot q_t=q_t-\Exv{v_{\pi(t)}\sim\Fi{t}}{\x{t}(v_{\pi(t)})}=q_{t+1}
\end{align*}
Next we claim that by conditioning the realized value at time $t$ to be $v$, the policy allocates the item with probability $\x{t}(v)$. This is simply true because the policy reaches time $t$ with probability $q_t$, and then conditioned on reaching time $t$ and realizing value $v$ allocates the item with probability $\frac{\x{t}(v)}{q_t}$. Finally, as $\{\x{t}(v)\}$ are the allocation probabilities of the policy (as we just proved), the expected allocated value at time $t$ is equal to $\Exv{v_{\pi(t)}\sim\Fi{\pi(t)}}{v_{\pi(t)}\cdot \x{t}(v_{\pi(t)})}$. The proof of the proposition is then finished by summing over all $t$.
\qed
\end{proof}

\subsection{Expected relaxation and rounding}
The goal of this section is to propose two sequential pricing policies, one for the case of non-identical distributions and one for the case of identical distributions, so that they obtain $\tfrac{1}{2}$ and $1-\tfrac{1}{e}$ fractions of the expected value of the omniscient prophet benchmark, respectively. To this end, we use \ref{eq:lp-opt-on} and the rounding algorithm proposed in \Cref{prop:rounding-exact}, and in a modular fashion design new algorithms satisfying the classic prophet inequality of \cite{krengel1978semiamarts} and the semi-optimal prophet inequality of \cite{correa2017posted} and \cite{esfandiari2017prophet}.


Our approach is based on the expected relaxation of \ref{eq:lp-opt-on}. Suppose the seller intends to sell the item, but rather than selling the item to only one buyer for every profile of buyer values, it has a relaxed constraint of selling the item to one person in expectation over buyer values. Without loss of generality, assume $\forall t:~\pi(t)=t$ (this will be cleared shortly). In the expected relaxation benchmark the seller only needs to sell the item to each buyer $t$ with probability $q_t$, where $\sum_t q_t\leq 1$. Clearly, the maximum expected value of the expected relaxation is an upper-bound on the expected value of the optimum offline mechanisms, as the omniscient prophet allocates the item to only one buyer point-wise. Moreover, the 
following linear program captures the expected relaxation:
\begin{align*}
\raisetag{70pt}
\label{eq:lp-ex-ante}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle \sum_{t=1}^{n}\Exv{v_{t}\sim\Fi{t}}{v_{t}\cdot \x{t}(v_{t})}  & &\tag{\texttt{Expected-LP}}\\
\text{subject to}& \displaystyle \sum_{t\in[n]}\Exv{v_{t}\sim\Fi{t}}{\x{t}(v_{t})} \leq 1,& \\
& \x{t}(v)\geq 0, &~~~~~~~\forall v\in \textrm{supp}(\Fi{t}),~t=1,\ldots,n
\end{array}
\end{align*}
Fix a feasible assignment $\{\x{t}(v)\}$ for the above LP, and let $q_t=\Exv{v_{t}\sim\Fi{t}}{\x{t}(v_{t})}$. Note that $\sum_t q_t\leq 1$. Now, one can replace $\{\x{t}(v)\}$ with the following assignment, which obtains at least as much expected value as before and is a feasible assignment for \ref{eq:lp-ex-ante}:
\begin{equation*}
\x{t}'(v)=
  \begin{cases}
       1 &\quad\quad\quad\quad   v\geq T_t(q_t),\\
       0 &\quad\quad\quad\quad\quad  \textrm{o.w.}
     \end{cases}
\end{equation*}



where $T_t(q_t)$ is the price corresponding to the quantile $q_t$ of the distribution $\Fi{t}$. More precisely, we define $T(q)\triangleq \underset{p\in \mathbb{R}}{\textrm{argmin}}~\mathbb{P}_{v\sim\mathcal{F}}\left[{v\geq p}\right]=q$. Under the pricing allocations $\{\x{t}'(v)\}$, the objective value of the expected LP is equal to $\sum_{t=1}^n V_t(q_t)$, where $V_t(q_t)$ is the concave value-curve of the distribution $\Fi{t}$. More precisely, we define $V(q)\triangleq \Exv{v\sim\mathcal{F}}{v\cdot \mathds{1}\{v \geq T(q)\}}$. By putting all the pieces together, the optimal solution to \ref{eq:lp-ex-ante} is $\x{t}^*(v)=\mathds{1}\{v\geq T_t(q^*_t)\}$, where $\mathbf{q}^*$ is the optimal solution of the following convex program:
\begin{align*}
\raisetag{70pt}
\label{eq:con-ex-ante}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle \sum_{t=1}^{n}V_t(q_t)& &\tag{\texttt{Expected-Conv}}\\
\text{subject to}& \displaystyle \sum_{t\in[n]}q_t\leq 1~,~q_t\geq 0&~~~~~~~t=1,\ldots,n
\end{array}
\end{align*}

\begin{remark} Note that the optimal solution of the expected relaxation (\ref{eq:lp-ex-ante}) can be computed by only knowing the set of distributions $\{\Fi{t}\}_{t\in [n]}$, and without the need to know the ordering $\pi$. In other words, this benchmark, similar to optimum offline, is \emph{order oblivious}; no matter what the ordering $\pi$ is, the expected relaxation yields the same solution.
\end{remark}

\paragraph{Rounding for the non-identical distributions.}
We now start with the optimal solution of the expected relaxation described above, i.e. $\{\x{t}^*(v)\}$, and modify it so that it becomes online implementable. In a nutshell, consider $\x{t}(v)=\tfrac{1}{2}\x{t}^*(v)$. We show this solution is feasible for \ref{eq:lp-opt-on}, for any $\pi$ as the true ordering of the buyers. Below, without loss of generality, assume $\forall t: \pi(t)=t$. 
\begin{proposition}The expected value obtained by Algorithm~\ref{alg:non-identical} is at least $\tfrac{1}{2}$ of optimum offline.
\end{proposition} 
\begin{proof}{Proof.}
Suppose $\x{t}^*(v)=\mathds{1}\{v\geq T_t(q^*_t)\}$ is the optimal assignment of (\ref{eq:lp-ex-ante}), where $\mathbf{q}^*$ is the optimal solution of the convex program \ref{eq:con-ex-ante}. Consider $\x{t}(v)=\tfrac{1}{2}\x{t}^*(v)$. We have:
\begin{equation*}
\x{t}(v)=\tfrac{1}{2}\x{t}^*(v)\overset{(1)}{\leq} \tfrac{1}{2}\overset{(2)}{\leq} 1-\tfrac{1}{2}\sum_{t'<t}q^*_{t'}\overset{(3)}{=}1-\Exv{v_{t'}\sim\Fi{t'}}{\x{t'}(v_{t'})}
\end{equation*}
where inequality~(1) holds as $\x{t}^*(v)\leq 1$, inequality~(2) holds as $\sum_{t'<t}q^*_{t'}\leq \sum_{t'}q^*_{t'}\leq 1$, and equality~(3) holds as $\Exv{v_{t'}\sim\Fi{t'}}{\x{t'}(v_{t'})}=\frac{1}{2}\Exv{v_{t'}\sim\Fi{t'}}{\x{t'}^*(v_{t'})}=\frac{1}{2}q^*_{t'}$. Therefore, $\{\x{t}(v)\}$ forms a feasible assignment for the \ref{eq:lp-opt-on}.\footnote{Note that we assume the true $\pi$ is the unitary ordering, but that is without loss of generality.}  By applying \Cref{prop:rounding-exact}, there exists a feasible randomized policy that implements $\{\x{t}(v)\}$; this policy obtains exactly the same allocation probabilities as $\{\x{t}(v)\}$ and obtains an expected value equal to the objective value of \ref{eq:lp-opt-on} for this assignment. Clearly, this objective value is at least $\frac{1}{2}$ of the expected value of the optimum offline, as the optimal value of the expected relaxation program is an upper-bound on the expected maximum value. Finally, note that the randomized policy implementing $\x{t}(v)$, described in the proof of \Cref{prop:rounding-exact}, is exactly equivalent to Algorithm~\ref{alg:non-identical}.
\qed
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[H]
\small
\caption{Online policy for non-identical distributions}
\begin{algorithmic}[1]
\State \textbf{input}: Distributions $\{\Fi{1},\ldots,\Fi{n}\}$
\State  Compute the optimal solution of (\ref{eq:con-ex-ante}). Let $\mathbf{q}^*$ be this optimal solution.
 $t\leftarrow 0$
\State \textbf{While} $\left(\left[~\textrm{item is not allocated}~\right]~\&~\left[ t\leq n \right]\right)$~\textbf{do}
 \State \quad\quad$t\leftarrow t+1$.
 \State \quad \quad Post a price $p_t\triangleq T_t(q^*_t)$.
 \State \quad \quad \textbf{If}~price $p_t$ gets accepted ($v_t\geq p_t$),~\textbf{then}
 \State  \quad\quad \quad\quad Allocate the item with probability $\displaystyle\frac{1}{2-\sum_{t'<t}q^*_{t'}}$.
\State \textbf{End}
\end{algorithmic}
\label{alg:non-identical}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{algorithm}[h]
%\small
%\caption{Online policy for non-identical distributions}
%\label{alg:non-identical}
%   \textbf{input}: Distributions $\{\Fi{1},\ldots,\Fi{n}\}$\\
% Compute the optimal solution of (\ref{eq:con-ex-ante}). Let $\mathbf{q}^*$ be this optimal solution. \em
% $t\leftarrow 0$\em
% 
% \textbf{while}~$\left(\left[~\textrm{item is not allocated}~\right]~\&~\left[ t\leq n \right]\right)$~\textbf{do}\em
% 
%$\large{\{}$\em
% 
% \quad\quad$t\leftarrow t+1$.\em
% 
% \quad\quad Post a price $p_t\triangleq T_t(q^*_t)$.\em
% 
% \quad\quad\textbf{if}~price $p_t$ gets accepted ($v_t\geq p_t$),~\textbf{then}~\em
% 
%  \quad\quad$\large{\{}$\em
%
% \quad\quad \quad\quad Allocate the item with probability $\displaystyle\frac{1}{2-\sum_{t'<t}q^*_{t'}}$. \em
% 
%  \quad\quad$\large{\}}$
% 
%$\large{\}}$
%\end{algorithm}
\paragraph{Rounding for the identical distributions.}
Can we round the optimal expected solution for the case of identical distributions, and obtain the improved bound of $1-\tfrac{1}{e}$, or even the optimal bound in \cite{correa2017posted}? Interestingly, by incorporating a careful rounding of the expected solution and using the LP of the optimum online, we can obtain a mechanism which is posting the single price of $T(\tfrac{1}{n})$ and show that it achieves at least $1-\tfrac{1}{e}$ fraction of the optimum offline (hence an alternative proof for a similar result in \cite{correa2017posted} and \cite{esfandiari2017prophet}). 

\begin{proof}{Proof.}
Due to the symmetry, the optimal solution of \ref{eq:con-ex-ante} is attained at $q^*_i=\tfrac{1}{n}$, and hence $\x{t}^*(v)=\mathds{1}\{v\geq T(\tfrac{1}{n})\}$. Let $\gamma\triangleq 1-\tfrac{1}{n}$, and consider the solution $\x{t}(v)=\gamma^t\cdot \x{t}^*(v)$. Note that $\Exv{v\sim\Fi{}}{\x{t}^*(v)}=\tfrac{1}{n}=1-\gamma$ for all $t$. Moreover, we have $\x{t}(v)=\gamma^t\cdot \x{t}^*(v)\leq \gamma^t$, simply because $\x{t}^*(v)\leq 1$. Therefore, 
\begin{equation*}
1-\sum_{t'<t}\Exv{v_{t'}\sim\Fi{}}{\x{t'}(v_{t'})}=1-\sum_{t'<t}\gamma^{t'}\cdot\Exv{v_{t'}\sim\Fi{}}{\x{t'}^*(v_{t'})}=1-\frac{1}{n}\frac{1-\gamma^t}{1-\gamma}=\gamma^t
\end{equation*}
where in the last equality we used $\gamma=1-\tfrac{1}{n}$. So, $\x{t}(v)\leq 1-\sum_{t'<t}\Exv{v_{t'}\sim\Fi{}}{\x{t'}(v_{t'})}$, and hence forms a feasible solution to \ref{eq:lp-opt-on} for any $\pi$. \Cref{prop:rounding-exact} suggests that there exists a randomized policy that implements this feasible assignment. In fact, similar to the proof of \Cref{prop:rounding-exact}, the final policy should post the price $T(\tfrac{1}{n})$, and if $v\geq T(\tfrac{1}{n})$ should accept it with probability:
\begin{equation*}
\displaystyle\frac{\gamma^t}{1-\sum_{t'<t}\Exv{v_{t'}\sim\Fi{}}{\x{t'}(v_{t'})}}=\frac{\gamma^t}{1-\frac{1}{n}\sum_{t'<t}\gamma^{t'}}=\frac{\gamma^t}{1-\frac{1}{n}\frac{1-\gamma^t}{1-\gamma}}=1,
\end{equation*}
where the last equality again holds because $\gamma=1-\tfrac{1}{n}$. So, the exact rounding policy simply suggests posting the single price $T(\tfrac{1}{n})$. To compare the expected value of this policy with that of the optimum offline, we only need to compare the objective value of \ref{eq:lp-opt-on} at this solution with the expected objective value, thanks to \Cref{prop:rounding-exact}. We have:
\begin{equation*}
\displaystyle \sum_{t=1}^{n}\Exv{v_{t}\sim\Fi{}}{v_{t}\cdot \x{t}(v_{t})}= \sum_{t=1}^{n}\gamma^t\cdot\Exv{v_{t}\sim\Fi{}}{v_{t}\cdot \mathds{1}\{v_t\geq T(\frac{1}{n})\}}=V(\frac{1}{n})\sum_{t=1}^n \gamma^t=V(\frac{1}{n})\frac{1-\gamma^{n+1}}{1-\gamma}~,
\end{equation*}
where the right-hand-side is equal to $n\cdot V(\tfrac{1}{n})\cdot (1-(1-\tfrac{1}{n})^{n+1})$ as $\gamma=1-\tfrac{1}{n}$. Finally, the expected optimal objective is equal to $n\cdot V(\tfrac{1}{n})$ and $(1-(1-\tfrac{1}{n})^{n+1})\geq 1-\frac{1}{e}$, which completes the proof.
\qed
\end{proof}


==> tex/abstract.tex <==
\begin{abstract}
We study online pricing algorithms for Bayesian online selection problems. Our goal is to find an adaptive pricing algorithm for serving a sequence of arriving buyers that maximizes the expected social welfare (or revenue) subject to different types of structural constraints. In this paper, we use the optimum online policy as a benchmark and in this sense we deviate from the prophet inequality framework which compares various policies to the omniscient prophet or equivalently the optimum offline. 

We first study the case where the allowable subsets of served customers are characterized by a laminar matroid with constant depth. This problem is a special case of the well-known matroid Bayesian online selection problem studied in \cite{kleinberg2012matroid}, when the underlying matroid is laminar. We give the first Polynomial-Time Approximation Scheme (PTAS) for the above problem. Our approach is based on rounding the solution of a hierarchy of linear programming relaxations that can approximate the optimum online solution with any degree of accuracy, as well as a concentration argument that shows that our rounding does not have a considerable loss in the expected social welfare. 

Next, we introduce the production constrained problem, for which the allowable subsets of served customers are characterized by joint production/shipping constraints that can be modeled by a special case of laminar matroids. We show that by leveraging the special structure of this problem and using a similar approach as before, \revcolor{we can design a polynomial-time approximation scheme for this problem, although in this special case the depth of the laminar matroid is not constant.} To achieve our result we exploit the negative dependency of the selection rule in the lower levels of the laminar family.
\end{abstract}


==> tex/intro-rad.tex <==
%----------------------------------
%Bayesian online selection, captures selling resources to rational agents
This paper revisits a canonical problem in revenue management: how should a planner allocate a limited number of goods or resources to a set of agents arriving over time? Applications of this problem include selling seats in a concert hall,  online retail, or sponsored-search auctions. 

In several of these applications, it is often reasonable to assume that each agent has a private valuation drawn from a known distribution. Moreover, the allocation is often subject to combinatorial constraints such as matroids, matchings, or knapsacks. The goal of the planner is to design online allocation mechanisms to maximize social welfare, i.e., the total value of served agents. This problem, termed as \emph{Bayesian online selection}, is originated from the seminal work of \citeauthor{krengel1978semi} in the 70s, and has since been studied  extensively (see \cite{lucier2017economic}, for a comprehensive survey). 
%The goal of the planner is then to design incentive compatible allocations (accompanying with right payments) to maximize social-welfare, i.e., the total value of served agents, or to maximize revenue, i.e., the total payments collected from agents. 

To understand the role of complex combinatorial constraints in applications of Bayesian online selection, consider a revenue management setting as follows. Suppose an airline is seeking to manage the  sale of flight itineraries. As a concrete example, suppose the airline focuses on flight requests with origin in \texttt{SFO}, first level connection (or destination) in \texttt{LAX}, \texttt{SEA}, and \texttt{ORD}, and second level connection (or destination) in \texttt{SAN} and \texttt{PHX} (through \texttt{LAX}), \texttt{YVR} and \texttt{YYC} (in Canada, through \texttt{SEA}) and \texttt{BNA}, \texttt{BUF} and \texttt{PIT} (through \texttt{ORD}). See \Cref{fig:map}. Passengers  with known value distributions request to book flights from \texttt{SFO} over time. Each passenger's request has a specific flight itinerary, e.g., $\texttt{SFO}\rightarrow \texttt{ORD}\rightarrow\texttt{PIT}$ or $\texttt{SFO}\rightarrow \texttt{LAX}$.  Suppose the airline considers a capacity for each airport on the number of served flight itinerary requests that are originated from \texttt{SFO}. These capacities are due to limitations such as number of crews, number of airport parking spots assigned to this airline, and cost of fuel in various airports. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=1\columnwidth]{FIG/map-red.pdf}
     \vspace{-1.2cm}
     \caption{The ``hierarchical'' map of airports in selling flight itineraries.}
      \label{fig:map}
\end{figure}

Now, the goal in the above example is to serve arriving requests (ideally by pricing the itineraries and serving those who are willing to pay the price) while respecting the airport capacities, so as to maximize revenue, which is equal to the total money collected from agents through pricing. Notably, in a single-parameter Bayesian setting like in this example, the problem of maximizing the revenue can also be reduced to the allocation problem of maximizing welfare with a simple transformation using (ironed) virtual values~\citep{myerson1981optimal}. Therefore, this example is indeed a Bayesian online selection problem with its specific combinatorial constraints due to the hierarchy of airports and their capacities, which we elaborate on more shortly.



%----------------------------------

% a key approach is "prophet inequality", it is amazing (many implications in mechanism design), simple, pricing, leads to approximations w.r.t. the prophet benchmark, information theoretically hard to pass barriers (like 1/2 for matroid Bayesian online selection)

A common approach to the above stochastic online optimization problem of Bayesian online selection, including the example of selling flight itineraries,  is to attain \emph{``prophet inequalities''}. In this approach, the goal is to evaluate the performance of an online algorithm relative to an offline ``omniscient  prophet'', who knows the valuation of each agent and therefore can easily maximize the social-welfare. The upshot of a significant line of work studying prophet inequalities is that in many complex combinatorial settings there exist simple and elegant take-it-or-leave-it pricing rules that obtain a constant factor approximation with respect to the omniscient prophet benchmark. Examples include (but are not limited to) single-item sale~\citep{samuel1984comparison, hill1982comparisons, correa2017posted}, matroids~\citep{hajiaghayi2007automated,chawla2010multi,kleinberg2012matroid}, matchings~\citep{chawla2010multi, alaei2012online,alaei2014bayesian,gravin2019prophet}, intersections of matroids~\citep{feldman2016online,ma2019algorithms}, and even combinatorial auctions~\citep{feldman2013simultaneous}. Somewhat surprisingly, it is also often possible to prove matching information theoretic lower-bounds (e.g. in matroids), i.e., showing that no online algorithm can obtain a better constant factor of the omniscient prophet than that of the simple pricing rules ~\citep{niazadeh2018prophet}.
%----------------------------------

%online stochastic optimization: why is important? mysterious computational complexity, PSPACE hardness for very general cases (MDP), not information theoretically hard (DP exists), computationally might or might not be tractable 
In this paper, we deviate from the above framework and dig into the question of characterizing and computing {\em optimum online policies}. Given the sequence of value distributions,   Bellman's ``principle of optimality''~\citep{bellman1954theory} proposes a simple dynamic programming that computes the optimum online policy for all of the above problems. Unfortunately, the dynamic program needs to track the full state of the system and therefore it often requires exponential time and space. 


%Moreover, no information theoretic lower-bounds stop an online policy to be as good as the optimum one, and in that sense our question is inherently computational. 


%----------------------------------
%approximations and PTAS, why is it better to approximate optimal online 

%While there are fairly strong lower bounds for the closely related computation of Markov Decision Processes (see  \cite{papadimitriou1987complexity} for the PSPACE-hardness of the general Markove decision processes with partial observations and XXX for EXPSPACE resutl.), the computational complexity of the online stochastic optimization problems with a concise combinatorial structure like the one we are considering here is poorly understood.

While there are fairly strong lower bounds for the closely related computation of Markov Decision Processes (see  \cite{papadimitriou1987complexity} for the PSPACE-hardness of the general Markov decision processes with partial observations), the computational complexity of the stochastic online optimization problems with a concise combinatorial structure, like the one we are considering here, is poorly understood.\footnote{To the best of our knowledge, there is no formal hardness result for this special class of stochastic online optimization, even for general matroid Bayesian online selection. This is indeed an interesting open problem.}
Here,  we ask whether it is possible to approximate the optimum online in polynomial time, and obtain improved approximation factors compared to those derived from the prophet inequalities. If we answer this question in the affirmative,  it justifies the optimum online policy as a less pessimistic benchmark compared to the omniscient prophet benchmark.


\subsection{Our main contributions}
We focus on two special cases of the Bayesian online selection problem.  First, inspired by the application of selling flight itineraries, we consider the problem of \emph{laminar Bayesian selection}. This problem is a special case of the well-known matroid Bayesian online selection problem studied in \cite{kleinberg2012matroid}, when the underlying matroid is laminar. In this problem, elements arrive over time with values drawn from heterogeneous but known independent distributions. A rooted directed  tree whose leaves are these elements and has a capacity on each of its internal nodes specifies the laminar matroid feasibility constraints as follows. For every internal node of the tree, a feasible set of elements (a.k.a. an independent set) does not include more leaves under this node (which are leaves that are connected to this node through a directed path) than its capacity (cf. the example of selling flight itineraries above and \Cref{fig:map}).  \cite{kleinberg2012matroid} show a tight $2$-approximation prophet inequality for this problem. Here, we focus on approximations to the optimum online policy instead.

Second, we consider another variation of laminar Bayesian selection interesting in its own right.  
Consider a firm producing (or receiving) multiple copies of different product types over time. The firm offers the products to arriving unit-demand buyers, where each buyer is interested in one product type and they have valuations drawn independently from known possibly non-identical distributions. The goal is to compute approximations to the optimum online policy for maximizing social-welfare (or revenue) subject to two constraints. First, at any time the total number of sold items of each type is no more than the number of produced items. Second, the total number of sold items does not exceed the total shipping capacity. We term this stochastic online optimization problem as \emph{production constrained Bayesian selection} .

%----------------------------------

%main results
We show both of these problems are amenable to polynomial time approximations with any degrees of accuracy. In a nutshell, our methodology is based on introducing linear programming relaxations for these problems and then designing appropriate rounding schemes through pricing.
\vspace{1mm}
\begin{displayquote}
\emph{\textbf{Main Results.} We give Polynomial Time Approximation Schemes (PTAS) for the laminar Bayesian selection problem when the depth of the laminar family is bounded by a constant, as well as the production constrained Bayesian selection problem.}
\end{displayquote}
\vspace{1mm}
As a subsidiary result, and also to further showcase our techniques in this paper, we extend our linear programming based approach to derive classic prophet inequality results known in the literature for the single-item Bayesian online selection problem~\citep{krengel1978semiamarts,hill1982comparisons,abolhassani2017beating,correa2017posted}. As a result, for the case of non-identical distributions we introduce a new adaptive pricing policy that obtains $\tfrac{1}{2}$ fraction of the expected value of the prophet benchmark. Moreover, for the case of identical distributions we show a simple single-price policy that obtains $(1-\tfrac{1}{e})$ fraction of the expected value of the prophet benchmark. To the best of our knowledge, this is the first use of linear programming techniques to obtain prophet inequalities in a modular fashion.
%----------------------------------

%motivating both problems through real-world examples (amazon, tesla, etc.)




%----------------------------------
%Our approach is based on a new LP for chracterizing feasible online policies, inspired by the natural DP, can be exactly rounded, but exponential-sized

\subsection{Overview of the techniques} We start by characterizing the optimum online policy for both of the problems through a \emph{Linear Programming} formulation. The LP formulations capture Bellman's dynamic program by tracking the state of the system through allocation and state variables (see \cref{sec:production-simple} for more details) and express the conditions for a policy to be \emph{feasible}  and \emph{online implementable} as linear constraints. Our method for capturing optimum online policy through linear programming resembles the dynamic programming to linear programming conversion technique introduced in \cite{de2003linear}. The resulting LPs are exponentially big but they accept polynomial-sized \emph{relaxations} with a small error. Furthermore, the relaxations can be rounded and implemented as online implementable policies, in the same way as exponential-sized LPs. 


%----------------------------------

% our remedy is relaxing the program, we propose that have polynomial-size LP

More precisely, we propose a hierarchy of linear programming relaxations that systematically strengthen the commonly used ``ex-ante'' LP formulation of  the problem and approximate the optimum solution with any degrees of accuracy. The first level of our LP hierarchy is the ex-ante relaxation, which is a simple linear program requiring that the allocation satisfies the capacity constraint(s) only in expectation. It is well-known that the integrality gap of this LP is 2~\citep{duetting2017prophet,alaei2014bayesian}.  At the other extreme, the linear program is of exponential size and is equivalent to the dynamic program. 



%----------------------------------
% for the first problem, either solve the ex-ante or the original LP,% we further generlize our approach to laminar; a hierarchy of linear programming relxations, can obtain desired accuracy at different 'levels' of the hierarchy (cutting the laminar tree)

Given $\eps$ as the error parameter of the desired PTAS, we show how to choose a linear program that combines the constraints of these two LPs in a careful way to get $\eps$-close to the optimum solution. In a nutshell, this hierarchy is parametrized by how we divide up the capacity constraints into ``large'' and ``small''.  In the laminar Bayesian selection, we consider the tree corresponding to the laminar family of constraints. Our approach here is based on chopping the tree (with the constraints as its internal nodes) by a horizontal cut, and then marking the constraints above the cut as large and below the cut as small (left figure, \Cref{fig:intro}). The final relaxation then needs to respect all the small constraints exactly and all the large constraints only in expectation.


\begin{figure}[ht]
  \centering
  \includegraphics[width=1\columnwidth]{FIG/intro-fig-red.pdf}
  \vspace{-0.8cm}
     \caption{Characterization of our hierarchy of linear programming relaxations.}
     \label{fig:intro}
\end{figure}
%----------------------------------
%rounding
Our final algorithms start by reducing the capacities of large bins by a factor of $(1-\eps)$ to create some slack, solve the corresponding LP relaxation, and then adaptively round the solution. A coupling argument shows that the LP solution can be implemented with an adaptive online pricing policy (potentially with randomized tie-breaking). However, the resulting online policy respects the large constraints only in expectation. 

In the production constrained Bayesian selection, we simply consider two cases based on shipping capacity being large or small (right figure, \Cref{fig:intro}). The main technical ingredient of the analysis for this algorithm is establishing {\em negative cylinder property} between the allocation events of this policy; this in turn leads to  concentration results on the number of allocated items in large bins (e.g. see~\citep{dubhashi1998balls}), and shows that the policy only violates the large capacity constraints with a small probability. 

The negative dependence analysis uses a very careful argument that essentially establishes  submodularity of the value function of the dynamic program.  See \cref{sec:production-simple} for the details. Surprisingly, the negative dependence property of optimum online policies no longer holds for laminar matroids with arbitrary arrival order of elements. We present examples in which the event that one agent accepts the offered price leads the optimum online to offer a lower price to the next agent!  In this case, we use a different trick by carefully chopping the laminar tree and marking the constraints to ensure negative dependence. See \Cref{sec:laminar} for the marking algorithm and its analysis. 



Finally, we focus on the classic single-item prophet inequality problem, where the ordering of buyers is unknown, but their values are independently drawn from known distributions. Inspired by the idea of hierarchy of linear programming relaxations used above, we consider two linear programs: ex-ante relaxation, in which the number of sold items in expectation is at most one, and the optimum online LP when the ordering is known. We first solve the ex-ante relaxation (which does not need to know the ordering of the buyers). Then, we show how to modify this optimal solution to be feasible in the optimum online LP. For the case of non-identical distributions, we introduce a modification that only loses $\tfrac{1}{2}$ of the ex-ante objective value, and for the case of identical distributions we introduce a new modification that only loses $\tfrac{1}{e}$ fraction of the ex-ante objective value. Interestingly, the resulting policies are order oblivious and are simple pricing policies (static for identical and adaptive for non-identical distributions) as mentioned earlier.

\input{tex/related.tex}


\subsection{Organization}

The rest of the paper is organized as follows. In \Cref{sec:laminar} we introduce the laminar matroid Bayesian selection problem and provide a PTAS for the case where the depth of the laminar matroid is constant. In \cref{sec:production-simple}, we formalize the production constrained Bayesian selection problem (which is a special case of the setting in \Cref{sec:laminar}) and show how we can leverage the structure of this problem to go beyond constant depth. We further showcase the applications of our linear programming based techniques for the single-item prophet inequality problem in \Cref{sec:lp-prophet}. Finally, we have the concluding remarks and future directions, along with a list of open questions, in \Cref{sec:conclusion}.



%Consider a production line producing a certain number of copies of an item everyday. During each day, heterogeneous customers arrive over time each with their own private valuations for the item. We consider a Bayesian setting where the customer values are drawn independently from known distributions. At the time of the arrival of a customer, we can offer her a price for the item which will result in a transaction if her valuation is bigger than or equal to the offered price. Our goal is to find a dynamic pricing mechanism that maximizes the expected social welfare,  which is the sum of the valuations of the agents who have received an item, in such a way that at any time the total number of items allocated to the customers is  no more than the number of produced items. 
%
%We call the above problem the {\em dynamic pricing for production constrained Bayesian selection}, or in short \emph{pricing with production constraints}. It is a special case of the well-known Bayesian online selection studied in \cite{kleinberg2012matroid}, also known as the matroid prophet inequality problem. In a Bayesian online selection problem, which was initiated by the seminal work of~\cite{krengel1978semiamarts}, the decision maker uses limited prior information, e.g. value distributions, to select a subset of elements arriving online. The selection is restricted to an underlying set system. In our problem, the set of customers arriving between day 1 and day $i$ for each $i$ form a nested family, each having a capacity that needs to be respected. Many variations of this problem are studied in which instead of the nested family with capacities the underlying set system is defined by  knapsack constraints~\citep{feldman2016online}, $k$-uniform matroids~\citep{hajiaghayi2007automated,alaei2014bayesian,chawla2010multi}, general matroids~\citep{kleinberg2012matroid,duetting2017prophet}, matchings~\citep{alaei2012online,bansal2012lp,feldman2009online,manshadi2012online} or beyond~\citep{rubinstein2016beyond}.
%
%We also study a generalization to laminar matroids. Consider a representation of the laminar family as a tree whose internal nodes are the \emph{bins} each with a given capacity, and the leaves are the \emph{elements}. The elements arrive over time, this time in an arbitrary but known order with valuations drawn independently from heterogeneous distributions. The goal is to pick a subset of elements with maximum possible total expected value while satisfying the capacity constraints. We assume the depth of the family (or equivalently the height of the tree) is bounded by a constant. 
%
%In the classic prophet inequality literature, the performance of a mechanism is typically evaluated relative to an ``omniscient prophet'', who knows the valuation of each agent and  therefore can easily maximize the social welfare. In that case, it is possible to prove information theoretic lower bounds showing one can not get better than a constant factor of the omniscient prophet. At the same time, there are several simple and elegant pricing rules that match the information  theoretic lower bound.
%
%This paper deviates from the above framework and tries to characterize {\em optimum online mechanisms}. For all the above problems, there is a simple dynamic program, also known as Bellman equation, that computes the optimum online pricing strategy. The dynamic program needs to track the full state of the system and therefore it often requires exponential time and space. We ask whether it is possible to approximate the optimum solution in polynomial time. In that sense, our question is inherently computational and in the realm of approximation algorithms. 
%
%We propose a hierarchy of linear programming relaxations that systematically strengthen the commonly used ``ex-ante'' linear programming formulation of  the problem and approximate the optimum solution with any degree of accuracy. The first level of our LP hierarchy is the ex-ante relaxation, which is a simple linear program requiring that the allocation satisfies the capacity constraint only in expectation. It is well-known that the integrality gap of this LP is 2~\citep{duetting2017prophet,alaei2014bayesian}, or in some cases $\frac{e}{e-1}$ (when pricing mechanism can change the ordering of the customers)~\citep{yan2011mechanism}.  At the other extreme, the linear program is of exponential size and is equivalent to the dynamic program. Given $\eps$, the error parameter of the polynomial-time approximation scheme, once can choose a linear program that combines the constraints of these two LPs in a careful way to get $\eps$-close to the optimum solution. 
%
%Our algorithm starts by reducing the capacities of large bins by a factor of $(1-\eps)$ to create some slack, solves the corresponding linear programming relaxation, and then adaptively rounds the solution. A coupling argument shows that the LP solution  can be implemented with a dynamic pricing mechanism (with randomized tie-breaking) that satisfies the production capacity corresponding to ``small bins'' exactly and the capacities of ``large bins'' in expectation.  The main technical ingredient of the analysis is establishing {\em negative cylinder dependency} between these  allocation events. The analysis uses very careful argument that essentially establishes  submodularity of the value function of the dynamic program. The negative cylinder dependency in turn leads to  concentration results on the number of allocated items in large bins. See \cref{sec:production-simple} for the details. 
%
%Surprisingly, the negative dependency no longer holds for laminar matroids. We present examples in which the event that one customer accepts the price offered to her leads the optimum online algorithm to a offer a lower price to the next customer!  In this case, we use a different family of linear programming relaxations, parameterized by different markings of bins into smalls and large. We refer the reader to \Cref{sec:laminar} for the algorithm and its analysis. 
%
%%Management of new products over time based on the demand of the market is critical for nearly all firms, and therefore has always been a quintessential focus of operations management~\citet{jermann1998asset}. With the prevalence of dynamic pricing mechanisms in electronic commerce, ride-sharing, airfare and many other modern platforms of trade, there has recently been a burst of interest in  integration of pricing mechanisms with production (or inventory)~\citet{deng2006joint}. Dynamic pricing is simple, easy-to-optimize, and strategy-proof against myopic users; nevertheless firms are bound with production constraints and their pricing scheme should meet these restrictions. 
%
%Online stochastic optimization problems arise naturally in a wide range of  pricing and matching applications. On one hand, management of the demand of the market is critical for nearly all firms and has always been a quintessential focus of operations management~\citep{jermann1998asset}. On the other hand, with the prevalence and growth of  electronic commerce platforms, online advertising markets, and ride-sharing apps, there has been a burst of interest in the computation of optimal (or near-optimal) matching and prices in real time. 
%
%However, recent models and algorithms for problems arising in these applications have focused on approximating the optimum offline solution ~(\citet{mehta2013online, mehta2007adwords, gupta2016algorithms, lucier2017economic, kleinberg2012matroid, manshadi2012online, feldman2009online}). As a result, we have very little understanding of the structure or complexity of the {\em optimum online solution}.  We hope that benchmarks similar to the type of linear programming hierarchy that we proposed here can lead to more insights and  new and interesting algorithms for this class of problems. 
%\begin{comment}
%\paragraph{More related work.} Beyond the traditional model of 
%
% 
% \begin{itemize}
% \item \citep{azar2014prophet}  k-uniform prophet inequity, if we only have access to one sample  from each distributions. They show how to get constant.
% \item an entire business of adaptivity gap, run by Anupam Gupta. I sent you the link to his talk SODA this year which I just found. I think we should somehow cite all of these papers:
% \citep{bhalgat2011improved} (stochastic knapsack)
% 
% \citep{ma2014improvements} (seems to be a PTAS for the above problem, but both in value and violation of the constraints)
% 
% \citep{gupta2016algorithms}
% 
% \end{itemize}
%\end{comment}
%
%  

==> tex/prelim.tex <==
\label{sec:twoone}
\label{sec:prob-desc}

Consider a production line producing $k_i$ items at the beginning of each day $i$ for $1 \leq i \leq L$.  During each day, a certain number of customers arrive over time in a given order and each customer is interested in obtaining at most one item. Each customer $t$ has a private valuation $v_t$ for the item which is a non-negative random variable drawn independently from a known discrete distribution $F_t$.   We are interested in an allocation mechanism that maximizes the expected social welfare, which is the sum of the valuations of the agents who have received an item,  in such a way that for any $i$, the number of elements allocated until the end of day $i$ is no more than $\sum_{j \leq i} k_j$. 

At the arrival of the $t^{\textrm{th}}$ customer, the mechanism can offer the customer a price $\tau_t$ for the item and the item is sold if $ v_t \geq \tau_t$. If the distributions are non-atomic the probability that $v_t = \tau_t$ is zero. Otherwise, the mechanism also determines the probability that the item is allocated to the agent if her value is equal to the offered price. 

We call the above problem  pricing for {\em Production Constrained Bayesian Selection}. Here is an equivalent formulation. Let $B_i$ be the set of customers arriving before the end of day $i$. $B_i$'s form set of $L$ nested bins, i.e., $B_1 \subseteq B_2 \subseteq \ldots \subseteq B_L$ with each bin $B_i$ having capacity $k_i$.  The elements corresponding to the customers arrive one by one in a given order such that all the elements in $B_1$ arrive first, then all the elements in $B_2 \setminus B_1$ arrive and so on. The $t^{\textrm{th}}$ arriving element has a value $v_t$ with a given distribution as before. Whenever an element arrives, one has to decide whether to pick or discard it based on its value. Our goal is to pick a subset respecting all capacity constraints such that the sum of the realized values in the subset is as large as possible in expectation. In \Cref{sec:nested}, we present a Polynomial Time Approximation Scheme (PTAS) for this problem. 

We will also consider a generalization to laminar families also known as the  \emph{Laminar Online Bayesian Selection} Problem. Consider a representation of the laminar family as a tree whose internal nodes are the \emph{bins} and the leaves are the \emph{elements}. The elements arrive over time, this time in an arbitrary but known order, and reveal their values. Each bin $i$ has a capacity $k_i$. The goal is to pick a subset of elements $1,2, \cdots, n$ with maximum possible total expected value, so that no more than $k_i$ elements are picked from each bin $i$.  We further assume values are drawn independently from known heterogeneous distributions. In \Cref{sec:laminar} we give a PTAS when the depth of the family (or equivalently the height of the tree) is constant. 

In both cases, we characterize the {\em optimum online pricing mechanism} and evaluate our algorithm against that benchmark. In that sense, we deviate from the prophet inequality framework that compares various mechanisms against the omniscient prophet or equivalently the optimum offline. It is not hard to see, and we will show this later, that these two benchmarks could be off by a factor 2 of each other even for very special cases. 


\begin{comment}
\subsection{Pricing with Nested Production and Laminar Resource Constraints}\label{sec:twotwo}
A scenario to portray this model would be to consider a factory producing different types of goods over a period of $L$ days. To make each good, we would need to produce its initial components and then assemble them together. Each type $t$ has a separate production line producing enough components to make $k_{t, i}$ goods of type $t$ in the first $i$ days. For each good, its components have to go through a series of assembly lines. The assembly lines of the factory have a hierarchical structure. More precisely, let $S_i$ denote the set of types than have to go through the $i^{\textrm{th}}$ assembly line. Then for any $i, j$, $S_i\subseteq S_j$, or $S_j\subseteq S_i$, or $S_i\cap S_j=\emptyset$. In addition, for any type $t$, if $t\in S_i$ and $S_i \subseteq S_j$, then goods of type $t$ go through the $i^{\textrm{th}}$ assembly line first.

We need to provide technical maintenance for each assembly line after processing a certain number of goods. Let $L_i$ denote the number of goods that can go through the $i^{\textrm{th}}$ assembly line before it needs maintenance. Customers arrive over days 1 through $L$ and are only interested in purchasing one good. The $t^{\textrm{th}}$ arriving customer offers a price $v_t$ for the good which is a nonnegative random variable, independently drawn from a known discrete distribution $F_t$. The order in which the consumers arrive and the types of goods they need is known in advance. The mechanism has to adaptively decide whether to accept or reject each offer, such that the welfare is maximized and for each type $t$, the number of sold goods of that type by the end of day $i$ is at most $k_{t, i}$. Furthermore, for each $i$, the total number of goods that go through the $i{\textrm{th}}$ assembly line has to be at most $L_i$.

\subsection{Laminar Matroid Online Bayesian Selection Problem}\label{sec:twothree}
Now we formally describe our model in the language of laminar matroids and the Bayesian online selection problem studied in \cite{kleinberg2012matroid}.

\begin{definition}[Laminar Matroid]
	Let $\mathcal{F}$ be a laminar family on set $S$ (i.e. if $X, Y \in \mathcal{F}$, then $X, Y \subseteq S$ and $X\subseteq Y$, or $Y\subseteq X$, or $X\cap Y=\emptyset$) such that each $x\in S$ is in some $X\in \mathcal{F}$. For each $X \in \mathcal{F}$ 
	there is a positive integer $k(X)$ associated with it. Let $\mathcal{I}=\set{I\subseteq S \given \lvert I\cap X\rvert \leq k(X), \forall X\in \mathcal{F}}$. Then $M=(\mathcal{I}, S)$ is a laminar matroid.
\end{definition}


Consider a laminar matroid $M=(\mathcal{I}, S)$. The elements in $S$ arrive one by one in a given order. Each element $e\in S$ has a value which is a nonnegative random variable with a known and discrete distribution $F_e$ which is realized upon arrival. Whenever the value of an arriving element is realized, one has to decide wether to pick or discard that element before the next element arrives. Our goal is to pick a feasible subset of elements $M \subseteq S$ that is independent, i.e. $M\in \mathcal{F}$ such that the sum of the realized values in $M$ is as large as possible.

One can see that this model is a more general case of the models described in \Cref{sec:twoone} and \Cref{sec:twotwo}.
\end{comment}

==> tex/proof-neg-dep.tex <==

We only need to show that the negative cylinder dependency holds for the dynamic programming that solves each sub-problem, as the distributions are non-atomic and there is a unique deterministic optimal online policy, characterized both by the LP and the dynamic programming. Consider sub-problem $j$. We use induction to show by serving more customers in the past, the prices for new buyers increase. Let $s_t^j$ denote the total number of products of type $j$ that have been sold up to the arrival of buyer $t$. Note that the algorithm only needs $s_t^j$ to decide whether buyer $t$ should be served.

Let $D_t(s_t^j)$ denote the maximum total expected welfare that an online policy can obtain from time $t$ to $n$, assuming that it starts from state $s_t^j$. Also let $C_t^j$ denote the set of production checkpoints of type $j$ that occur at or after time $t$.
	Using the Bellman equations we have	
\[   
D_{t-1}(s_{t-1}^j) = 
   \left\{
     \begin{array}{@{}l@{\thinspace}l}
       D_t(s_{t-1}^j)    &~~\textrm{if}~~ \min\left(\left\{k_i^j-s_{t-1}^j\right\}_{i\in C_{t-1}^j}\right)=0\\
       \Exv{v_{t-1}}{\max(D_t(s_{t-1}^j+1)+v_{t-1}, D_t(s_{t-1}^j))} &~~\textrm{if}~~ \min\left(\left\{k_i^j-s_{t-1}^j\right\}_{i\in C_{t-1}^j}\right)>0 \\
     \end{array}
   \right.
\]


As the base of our induction, we know that if we serve the last buyer, the probability that we serve any other buyers does not increase. Now assume while serving buyer $t$, we have
\begin{align}\label{inductionHypo}
	D_t(s_t^j)-D_t(s_t^j+1)\leq D_t(s_t^j+1)-D_t(s_t^j+2).
\end{align}
Note that this shows the price offered to buyer $t$ increases if we serve more buyers before buyer $t$.
When buyer $t-1$ arrives, we need to show
\begin{align}\label{inductionStep}
	D_{t-1}(s_{t-1}^j)-D_{t-1}(s_{t-1}^j+1)\leq D_{t-1}(s_{t-1}^j+1)-D_{t-1}(s_{t-1}^j+2)
\end{align}
which is equivalent to
$$D_{t-1}(s_{t-1}^j)+D_{t-1}(s_{t-1}^j+2)\leq 2D_{t-1}(s_{t-1}^j+1).$$
Note that this property is linear in the terms involved. So it is enough to assume that the value $v_{t-1}$ is deterministic first and prove the above inequality. Then by linearity of expectation, the inequality would hold in the general case.



Note that for the case where $\min\left(\left\{k_i^j-s_{t-1}^j\right\}_{i\in C_{t-1}^j}\right)<2$, the inequality holds trivially because we assume $D_{t-1}(s)=-\infty$ for any non-negative integer $s$ such that $\min\left(\left\{k_i^j-s\right\}_{i\in C_{t-1}^j}\right)<0$.
According to our induction hypothesis, if $D_{t-1}(s_{t-1}^j+2)$ is updated, then the other two variables are updated as well. More precisely, if $D_{t-1}(s_{t-1}^j+2)=D_t(s_{t-1}^j+3)+v_{t-1}$, then
\begin{align*}
	&D_{t-1}(s_{t-1}^j+1)=D_t(s_{t-1}^j+2)+v_{t-1},\\
	&D_{t-1}(s_{t-1}^j)=D_t(s_{t-1}^j+1)+v_{t-1}.
\end{align*}
In a similar way, if $D_{t-1}(s_{t-1}^j+1)=D_t(s_{t-1}^j+2)+v_{t-1}$, then
\begin{align*}
	D_{t-1}(s_{t-1}^j)=D_t(s_{t-1}^j+1)+v_{t-1}.
\end{align*}

Considering these relations, we have three different cases. (i) none of these variables are updated. In this case, \cref{inductionStep} turns into \cref{inductionHypo} which holds according to our induction hypothesis. (ii) all of these variables are updated. In this case, \cref{inductionStep} turns into
\begin{align*}
	D_t(s_t^j+1)+v_{t-1}-D_t(s_t^j+2) - v_{t-1} \leq D_t(s_t^j+2) + v_{t-1} - D_t(s_t^j+3) - v_{t-1}
\end{align*}
which holds again according to the induction hypothesis.
Finally, (iii) the case where $D_{t-1}(s_{t-1}^j)$ is updated and $D_{t-1}(s_{t-1}^j+2)$ is not updated. In this case, we can write \cref{inductionStep} as
\begin{align*}
	D_t(s_t^j+1)+v_{t-1}+D_t(s_t^j+2)\leq 2 \max(D_t(s_t^j+2)+v_{t-1}, D_t(s_t^j+1))
\end{align*}
and this always holds because for any two values $x, y$, $\frac{x+y}{2}\leq \max(x, y)$.
\end{proof}


\subsection{Discussion: extension to laminar over non-constant depth sub-problems.}
As we saw earlier in \Cref{sec:laminar-mark}, we can prove the correctness of our polynomial time approximation scheme for general laminar matroids only if the depth of the laminar family is constant. At the same time, as an observation, if one thinks of the production constrained Bayesian selection problem as an instance of the laminar Bayesian selection, then the depth of the corresponding laminar family will simply be $T+1$, and hence is not a constant. Yet, as we saw, our approach in \cref{sec:production-simple} could also yield a PTAS. Can we still see this PTAS as a special case of our PTAS for the constant-depth laminar?

This discrepancy can easily be explained by extending our result for the constant depth laminar Bayesian selection to a generalization where every element is replaced by a \emph{sub-problem}. With this view, in the production constrained Bayesian selection we indeed have only a 1-level tree (connecting the root to the type-specific sub-problems), and each leaf of this 1-level tree plays the role of one of the type-specific sub-problems. To make the analysis work, we require two things from each sub-problem. First, a local optimum online policy for each sub-problem, for possibly atomic or even non-positive value distributions, should be computable in polynomial time. Second, the selection rule of this local optimum online policy should satisfy the required negative cylinder dependency. Having these two properties, the proof of this section goes through, as by replacing each element with a group of negatively dependent elements we still have the required concentration. The proof of this generalization is basically the same, and so we omit to avoid redundancy.


%We only need to show that the negative cylinder dependency holds for the dynamic programming that solves sub-problems $j$, as the distributions are non-atomic and there is a unique deterministic optimal online policy, characterized both by the LP and the dynamic programming. We use induction to show by serving more buyers in the past, the prices for new buyers increase. We assume, without loss of generality, that each buyer $t$ is contained in a bin $B_t$. Because if this is not the case, namely buyer $t$ and $t-1$ are in the same bin $B_{l_{t-1}}$, we can assume a new bin over buyers $t, t+1, \ldots, n$ with the same capacity as that of $B_{l_{t-1}}$. Let $\vec{r}$ be the vector of remaining capacities when buyer $t$ arrives (in bin $t$). Note that the algorithm only needs $r_i$ for $i\geq t$ to decide whether buyer $t$ should be served. We abuse notation and use $\vec{r}$ to also denote $[r_t, \ldots, r_n]$, wherever the index $t$ is clear from the context. Let $D_t(\vec{r})$ denote the maximum total expected  welfare that an online policy can obtain from time $t$ to $n$, assuming that it starts from remaining capacities $\vec{r}$.
%%	in  We consider two different cases. If buyer $t-1$ is in $B_{l_t}$, then we have:
%%	
%%	$$D_{t-1}(\vec{r})=\max(D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}))$$
%%	
%%	On the other hand, if buyer $t-1$ is in $B_{l_t-1}$, we have:
%	Using the Bellman equations we have:
%	\[   
%D_{t-1}(c, \vec{r}) = 
%   \left\{
%     \begin{array}{@{}l@{\thinspace}l}
%       D_t(\vec{r})    &~~\textrm{if}~~ \min\left({c,\{r_i\}}\right)=0\\
%       \Exv{v_{t-1}}{\max(D_t(\vec{r}-\vec{u_t})+v_{t-1}, D_t(\vec{r}))} &~~\textrm{if}~~ \min\left({c,\{r_i\}}\right)\geq 1 \\
%     \end{array}
%   \right.
%\]
%
%As the base of our induction, we know that if we serve the last buyer, the probability that we serve any other buyers does not increase. Now assume while serving buyer $t$, we have:
%\begin{align}\label{inductionHypo}
%	D_t(\vec{r})-D_t(\vec{r}-\vec{u_t})\leq D_t(\vec{r}-\vec{u_t})-D_t(\vec{r}-2\vec{u}_t)
%\end{align}
%Note that this shows the price offered to buyer $t$ increases if we serve more buyers before buyer $t$; this is because the effect of serving any buyer before $t$ on the remaining capacities is $u_t$.
%
%When buyer $t-1$ arrives, we need to show:
%\begin{align}\label{inductionStep}
%	D_{t-1}(c, \vec{r})-D_{t-1}(c-1, \vec{r}-\vec{u}_t)\leq D_{t-1}(c-1, \vec{r}-\vec{u}_t)-D_{t-1}(c-2, \vec{r}-2\vec{u}_t)
%\end{align}
%Which is equivalent to:
%$$D_{t-1}(c, \vec{r})+D_{t-1}(c-2, \vec{r}-2\vec{u}_t)\leq 2D_{t-1}(c-1, \vec{r}-\vec{u}_t)$$
%Note that this property is linear in the terms involved. So it is enough to assume that the value $v_{t-1}$ is deterministic first and prove the above inequality. Then by linearity of expectation, the inequality would hold in the general case.
%
%Note that for the case where $\min\left({c,\{r_i\}}\right)<2$, the inequality holds trivially because we assume $D_t(\vec{r})=-\infty$ if $\min\left(\{r_i\}\right)<0$.
%According to our induction hypothesis,  if $D_{t-1}(c-2, \vec{r}-2\vec{u}_t)$ is updated, then the other two variables are updated as well. More precisely, if $D_{t-1}(c-2, \vec{r}-2\vec{u}_t)=D_t(\vec{r}-3\vec{u}_t)+v_{t-1}$, then
%\begin{align*}
%	&D_{t-1}(c-1, \vec{r}-\vec{u}_t)=D_t(\vec{r}-2\vec{u}_t)+v_{t-1},\\
%	&D_{t-1}(c, \vec{r})=D_t(\vec{r}-\vec{u}_t)+v_{t-1}
%\end{align*}
%In a similar way, if $D_{t-1}(c-1, \vec{r}-\vec{u}_t)=D_t(\vec{r}-2\vec{u}_t)+v_{t-1}$, then
%\begin{align*}
%	D_{t-1}(c, \vec{r})=D_t(\vec{r}-\vec{u}_t)+v_{t-1}
%\end{align*}
%
%Considering these relations, we have three different cases. (i) none of these variables are updated. In this case, \Cref{inductionStep} turns into \Cref{inductionHypo} which holds according to our induction hypothesis. (ii) all of these variables are updated. In this case, \Cref{inductionStep} turns into
%\begin{align*}
%	D_t(\vec{r}-\vec{u}_t)+v_{t-1}-D_t(\vec{r}-2\vec{u}_t) - v_{t-1} \leq D_t(\vec{r}-2\vec{u}_t) + v_{t-1} -D_t(\vec{r}-3\vec{u}_t) - v_{t-1}
%\end{align*}
%which holds again according to the induction hypothesis.
%Finally, (iii) the case where $D_{t-1}(c, \vec{r})$ is updated and $D_{t-1}(c-2, \vec{r}-2u_t)$ is not updated. In this case, we can write \ref{inductionStep} as:
%\begin{align*}
%	D_t(\vec{r}-\vec{u}_t)+v_{t-1}+D_t(\vec{r}-2\vec{u}_t)\leq 2 \max(D_t(\vec{r}-2\vec{u}_t)+v_{t-1}, D_t(\vec{r}-\vec{u}_t))
%\end{align*}
%And this always holds because for any two values $x, y$, $\frac{x+y}{2}\leq \max(x, y)$.
%\end{proof}
%
%
%
%
%
%%If we expand the terms we have:
%%
%%\begin{align*}
%%	&\max(D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}))-\max(D_t(\vec{r}-2\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}}))\leq\\ 
%%	&\max(D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})+v_{t-1}, D_t(\vec{r}-\vec{u_j}))-\max(D_t(\vec{r}-2\vec{u_{l_t}}-\vec{u_j})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j}))
%%\end{align*}
%%
%%Now we consider three cases:
%%
%%Case 1: $D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})\geq D_t(\vec{r}-2\vec{u_{l_t}}-\vec{u_j})+v_{t-1}$ and $D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}\geq D_t(\vec{r})$
%%
%%For this case we have:
%%\begin{align*}
%%	&\max(D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}))-\max(D_t(\vec{r}-2\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}}))=
%%		\\&D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}-\max(D_t(\vec{r}-2\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}})) \leq 
%%		\\&D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}-D_t(\vec{r}-\vec{u_{l_t}}) \leq D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})+v_{t-1}-D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j}) \leq 
%%		\\&\max(D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})+v_{t-1}, D_t(\vec{r}-\vec{u_j}))-\max(D_t(\vec{r}-2\vec{u_{l_t}}-\vec{u_j})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j}))
%%\end{align*}
%%Case 2: $D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})\leq D_t(\vec{r}-2\vec{u_{l_t}}-\vec{u_j})+v_{t-1}$ and $D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}\geq D_t(\vec{r})$
%%For this case we have:
%%\begin{align*}
%%	&\max(D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}))-\max(D_t(\vec{r}-2\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}}))=
%%		\\&D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}-\max(D_t(\vec{r}-2\vec{u_{l_t}})+v_{t-1}, D_t(\vec{r}-\vec{u_{l_t}})) \leq 
%%		\\&D_t(\vec{r}-\vec{u_{l_t}})+v_{t-1}-D_t(\vec{r}-\vec{u_{l_t}}) \leq D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j})+v_{t-1}-D_t(\vec{r}-\vec{u_{l_t}}-\vec{u_j}) \leq
%%		\\&
%%\end{align*}
%%
%%When buyer $t-1$ is in $B_{l_t}-1$, we need to show:
%%$$D_{t-1}(c, \vec{r})-D_{t-1}(c-1, \vec{r}-\vec{u_{l_t}})\leq D_{t-1}(c, \vec{r}-\vec{u_j})-D_{t-1}(c-1, \vec{r}-\vec{u_{l_t}}-\vec{u_j})$$
%%
%%Again we begin by expanding the terms. We have to consider two different cases (i) When $c=1$ and (ii) when $c> 2$

